HAT-P-67b: An Extremely Low Density Saturn Transiting an F-Subgiant Confirmed via Doppler Tomography

We report the discovery of HAT-P-67b, a hot-Saturn transiting a rapidly rotating F-subgiant. HAT-P-67b has a radius of Rp = 2.085 -0.071/+0.096 RJ,, orbiting a M* = 1.642 -0.072/+0.155 Msun, R* = 2.546 -0.084/+0.099 Rsun host star in a ~4.81-day period orbit. We place an upper limit on the mass of the planet via radial velocity measurements to be Mp < 0.59 MJ, and lower limit of > 0.056 MJ by limitations on Roche lobe overflow. Despite being a subgiant, the host star still exhibits relatively rapid rotation, with a projected rotational velocity of v sin I* = 35.8 +/- 1.1 km/s, making it difficult to precisely determine the mass of the planet using radial velocities. We validated HAT-P-67b via two Doppler tomographic detections of the planetary transit, which eliminated potential eclipsing binary blend scenarios. The Doppler tomographic observations also confirmed that HAT-P-67b has an orbit that is aligned to within 12 degrees, in projection, with the spin of its host star. HAT-P-67b receives strong UV irradiation, and is amongst the one of the lowest density planets known, making it a good candidate for future UV transit observations to search for an extended hydrogen exosphere.

==> RV.tex <==
\begin{deluxetable*}{rrrrr}
\tablewidth{0pc}
\tabletypesize{\scriptsize}
\tablecaption{
       KECK-HIRES relative radial velocities and bisector span measurements of \hatcur{}
    \label{tab:rv_table}
}
\tablehead{
    \multicolumn{1}{c}{BJD}          &
    \multicolumn{1}{c}{RV}\tablenotemark{a}             &
    \multicolumn{1}{c}{$\sigma$ RV}      &
    \multicolumn{1}{c}{BS}         &
    \multicolumn{1}{c}{$\sigma$ BS}            \\
    \multicolumn{1}{c}{(UTC)} &
    \multicolumn{1}{c}{$(\mathrm{m\,s}^{-1})$} &
    \multicolumn{1}{c}{$(\mathrm{m\,s}^{-1})$} &
    \multicolumn{1}{c}{$(\mathrm{m\,s}^{-1})$} &
    \multicolumn{1}{c}{$(\mathrm{m\,s}^{-1})$}
}
\startdata
2455696.8366 & -105 & 28 & 24 & 11 \\ 
 2455696.88382 & -151 & 31 & 67 & 17 \\ 
 2455697.833 & 31 & 25 & -58 & 9 \\ 
 2455698.92918 & 93 & 23 & -53 & 8 \\ 
 2455699.83162 & 63 & 25 & 46 & 10 \\ 
 2455700.88206 & 1 & 22 & 30 & 13 \\ 
 2455704.84352 & 18 & 23 & -2 & 13 \\ 
 2455705.86007 & 100 & 22 & -34 & 8 \\ 
 2455706.83882 & 8 & 22 & 14 & 11 \\ 
 2455707.85238 & 35 & 22 & -17 & 13 \\ 
 2455853.70871 & -6 & 28 & ... & ... \\ 
2455945.15236 & -89 & 24 & ... & ... \\ 
2455997.02884 & -17 & 38 & ... & ... \\ 
2455017.0082 & 58 & 22 & ... & ... \\ 
2455042.88956 & -65 & 26 & ... & ... \\ 
2455043.9989 & -25 & 29 & ... & ... \\ 
2455044.94822 & -63 & 26 & ... & ... \\ 
2455048.86097 & -112 & 30 & ... & ... \\ 
2455107.71733 & 241 & 40 & -3 & 28 \\ 
[-1.5ex]
\enddata 
\tablenotetext{a}{
%%
 Internal errors excluding the component of astrophysical/instrumental jitter considered in Section 3. Bisector spans (BS) are given where available.
%%
}

\end{deluxetable*}

==> lc.tex <==
% \begin{table}
%   \caption{\label{lc_table}Differential photometry of \hatcur{}}
%   \begin{tabular}{rrrrr}
%     \hline\hline
%     BJD (UTC) & Flux$^a$ & $\Delta$Flux & Filter & Instrument \\
%     \hline




\begin{deluxetable*}{rrrrrrr}

\tablewidth{0pc}
\tabletypesize{\scriptsize}
\tablecaption{
        Differential photometry of \hatcur{}
    \label{tab:lc_table}
}
\tablehead{
    \multicolumn{1}{c}{BJD}          &
    \multicolumn{1}{c}{Mag (Raw)}\tablenotemark{a}             &
    \multicolumn{1}{c}{Mag (EPD)}            &
    \multicolumn{1}{c}{Mag (TFA)}            &
    \multicolumn{1}{c}{$\sigma$ Mag}      &
    \multicolumn{1}{c}{Instrument}         &
    \multicolumn{1}{c}{Filter}            \\
    &
    &
    &
    &
}
\startdata

2454521.99042 & 9.39859 & 9.72414 & 9.72271 & 0.00303& HATNet & R\\
2454521.99445 & 9.39572 & 9.72048 & 9.73067 & 0.00325& HATNet & R\\
2454521.99854 & 9.39262 & 9.72005 & 9.71695 & 0.00276& HATNet & R\\
2454522.00264 & 9.38941 & 9.7199 & 9.72327 & 0.00344& HATNet & R\\
2454522.00673 & 9.41475 & 9.74011 & 9.73327 & 0.00328& HATNet & R\\

% 2453385.02669 & 0.9983 & 0.0077 & $I$ & HAT\\
% 2453385.03421 & 1.0022 & 0.0061 & $I$ & HAT\\
% 2453385.03798 & 1.0082 & 0.0051 & $I$ & HAT\\
% 2453385.04189 & 0.9905 & 0.0044 & $I$ & HAT\\
% 2453385.04566 & 0.9994 & 0.005 & $I$ & HAT\\
% 2453385.04943 & 1.0013 & 0.0052 & $I$ & HAT\\
% 2453385.05321 & 1.0031 & 0.0046 & $I$ & HAT\\
% 2453385.05711 & 1.008 & 0.0045 & $I$ & HAT\\
% 2453386.02633 & 1.0143 & 0.003 & $I$ & HAT\\
% 2453386.03389 & 0.9813 & 0.0029 & $I$ & HAT\\
[-1.5ex]
\enddata 
\tablenotetext{a}{
%%
This table is available in a machine-readable form in the online journal. A portion is shown here for guidance regarding its form and content.\\
Raw, EPD, and TFA magnitudes are presented for HATNet light curves. The detrending and potential blending may cause the HATNet transit to be shallower than the true transit in the EPD and TFA lgiht curves. This is accounted for in the global modelling by the inclusion of a third light factor. Follow-up light curves have been treated with EPD simultaneous to the transit fitting. Pre-EPD magnitudes are presented for the follow-up light curves.

% This table is available in a machine-readable form in the online journal. A portion is shown here for guidance regarding its form and content.\\
% HATNet fluxes (HAT) have been treated with EPD and TFA prior to the transit fitting. The detrending and potential blending may cause the HATNet transit to be shallower than the true transit. This is accounted for in the global modelling by the inclusion of a third light factor. Follow-up light curves have been treated with EPD simultaneous to the transit fitting. Pre-EPD magnitudes are presented for the follow-up light curves.
%%
}

\end{deluxetable*}


==> newcommand_gen.tex <==
%%GB: General commands to make editing easier and with less typos.

%% -----------------------------------------------
%% Editing
\newcommand{\tbd}[1]{{\par\bf\textsc{TBD: #1\\}}}
\newcommand{\ctbd}[1]{}
\newcommand{\cor}{\textcolor{red}{(corr?) }}
\newcommand{\spl}{\textcolor{red}{(spl?) }}

%% ------------------------------------------------
%% Hun characters
\newcommand{\ii}{\'\i }
\newcommand{\oo}{\H{o}}
\newcommand{\uu}{\H u}

%% --------------------------------------
%% Often used. 
\newcommand{\lc}{light curve}
\newcommand{\lcs}{light curves}
\newcommand{\Lc}{Light curve}
\newcommand{\Lcs}{Light curves}
\newcommand{\avg}[1]{\ensuremath{\langle #1\rangle}}
\newcommand{\med}[1]{\ensuremath{\langle #1\rangle_{med}}}
\newcommand{\dpt}{data-point}
\newcommand{\dpts}{data-points}
\newcommand{\tel}{telescope}
\newcommand{\magn}{magnitude}
\newcommand{\stan}{standard}
\newcommand{\aper}{aperture}
\newcommand{\oot}{out-of-transit}
\newcommand{\OOT}{Out-of-Transit}
\newcommand{\cfa}{Harvard-Smithsonian Center for Astrophysics (CfA)}
\newcommand{\cfadigi}{CfA Speedometers}
\newcommand{\cmd}{color-magnitude diagram}

%% ---------------------------------------------
%% 
\newcommand{\conc}[1]{\noindent\par{\noindent{$\mathbf \Longrightarrow$ \bf #1}}}
\newcommand{\diam}{\ensuremath{\oslash}}
\newcommand{\ccdsize}[1]{\ensuremath{\rm #1\times\rm#1}}
\newcommand{\fovsize}[2]{\ensuremath{\rm #1 #2\times\rm#1 #2}}
\newcommand{\tsize}[1]{\mbox{\rm #1 m}}
\newcommand{\band}[1]{\ensuremath{#1}-band}
\newcommand{\ordo}{\ensuremath{\mathcal{O}}}
\newcommand{\chisq}{\ensuremath{\chi^2}}
\newcommand{\RA}[3]{\ensuremath{#1^{\mathrm h}#2^{\mathrm m}#3^{\mathrm s}}}
\newcommand{\DEC}[3]{\ensuremath{#1^{\mathrm d}#2^{\mathrm m}#3^{\mathrm s}}}

%% ---------------------------------------------------------------------
%% Dimensions/quantities
\newcommand{\ghr}{\ensuremath{^h}}
\newcommand{\gmin}{\ensuremath{^m}}
\newcommand{\Ks}{\ensuremath{K_s}}
\newcommand{\masy}{\ensuremath{\rm mas\,yr^{-1}}}
\newcommand{\kms}{\ensuremath{\rm km\,s^{-1}}}
\newcommand{\ms}{\ensuremath{\rm m\,s^{-1}}}
\newcommand{\mss}{\ensuremath{\rm m\,s^{-2}}}
\newcommand{\gcmc}{\ensuremath{\rm g\,cm^{-3}}}
\newcommand{\ergscmsq}{\ensuremath{\rm erg\,s^{-1}\,cm^{-2}}}
\newcommand{\C}{\ensuremath{^{\circ}C\;}}
\newcommand{\el}{\ensuremath{e^-}}
\newcommand{\sqarcsec}{\ensuremath{\Box^{\prime\prime}}}
\newcommand{\sqarcdeg}{\ensuremath{\Box^{\circ}}}
\newcommand{\pxs}{\ensuremath{\rm \arcsec pixel^{-1}}}
\newcommand{\aduel}{\ensuremath{\lbrack ADU/\el \rbrack}}
\newcommand{\eladu}{\ensuremath{\lbrack \el/ADU \rbrack}}
\newcommand{\adupixs}{\ensuremath{\rm ADU/(pix\, s)}}
\newcommand{\elpixs}{\ensuremath{\rm \el/(pix\, s)}}
\newcommand{\masyr}{\ensuremath{\rm mas\,yr^{-1}}}

%% ---------------------------------------------------------------------
%% General
\newcommand{\msini}{\ensuremath{m \sin i}}
\newcommand{\mplsini}{\ensuremath{\mpl\sin i}}
\newcommand{\teff}{\ensuremath{T_{\rm eff}}}
\newcommand{\logg}{\ensuremath{\log{g}}}
\newcommand{\vsini}{\ensuremath{v \sin{i}}}
\newcommand{\feh}{\ensuremath{\rm [Fe/H]}}
\newcommand{\logl}{\ensuremath{\log{L}}}
\newcommand{\vmac}{\ensuremath{v_{\rm mac}}}
\newcommand{\vmic}{\ensuremath{v_{\rm mic}}}
% Activity index R'_HK
\newcommand{\rhk}{\ensuremath{R^{\prime}_{HK}}}
% log of R'_HK
\newcommand{\logrhk}{\ensuremath{\log\rhk}}
% S average value
\newcommand{\Savg}{\ensuremath{\langle S\rangle}}


%% ---------------------------------------------------------------------
%% Solar quantities 
\newcommand{\rsun}{\ensuremath{R_\sun}}
\newcommand{\msun}{\ensuremath{M_\sun}}
\newcommand{\lsun}{\ensuremath{L_\sun}}
\newcommand{\loglsun}{\ensuremath{\log{L_\sun}}}
\newcommand{\teffsun}{\ensuremath{T_{eff,\sun}}}
\newcommand{\rhosun}{\ensuremath{\rho_\sun}}
\newcommand{\loggsun}{\ensuremath{\log{g_{\sun}}}}

%% ---------------------------------------------------------------------
%% Stellar quantities 
\newcommand{\rstar}{\ensuremath{R_\star}}
\newcommand{\mstar}{\ensuremath{M_\star}}
\newcommand{\lstar}{\ensuremath{L_\star}}
\newcommand{\astar}{\ensuremath{a_\star}}
\newcommand{\loglstar}{\ensuremath{\log{L_\star}}}
\newcommand{\teffstar}{\ensuremath{T_{\rm eff\star}}}
\newcommand{\rhostar}{\ensuremath{\rho_\star}}
\newcommand{\loggstar}{\ensuremath{\log{g_{\star}}}}

%% ---------------------------------------------------------------------
%% Earth
\newcommand{\rearth}{\ensuremath{R_\earth}}
\newcommand{\mearth}{\ensuremath{M_\earth}}
\newcommand{\learth}{\ensuremath{L_\earth}}
\newcommand{\teffearth}{\ensuremath{T_{\rm eff,\earth}}}
\newcommand{\rhoearth}{\ensuremath{\rho_\earth}}

%% ---------------------------------------------------------------------
%% Planetary
\newcommand{\rpl}{\ensuremath{R_{p}}}
\newcommand{\mpl}{\ensuremath{M_{p}}}
\newcommand{\lpl}{\ensuremath{L_{p}}}
\newcommand{\teffpl}{\ensuremath{T_{\rm eff,{p}}}}
\newcommand{\rhopl}{\ensuremath{\rho_{p}}}
\newcommand{\ipl}{\ensuremath{i_{p}}}
\newcommand{\epl}{\ensuremath{e_{p}}}
\newcommand{\gpl}{\ensuremath{g_{p}}}
\newcommand{\loggpl}{\ensuremath{\log g_{p}}}

\newcommand{\arstar}{\ensuremath{a/\rstar}}
\newcommand{\zrstar}{\ensuremath{\zeta/\rstar}}

%% ---------------------------------------------------------------------
%% Jupiter
\newcommand{\rjup}{\ensuremath{R_{\rm J}}}
\newcommand{\mjup}{\ensuremath{M_{\rm J}}}
\newcommand{\ljup}{\ensuremath{L_{\rm J}}}
\newcommand{\teffjup}{\ensuremath{T_{eff,{\rm J}}}}
\newcommand{\rhojup}{\ensuremath{\rho_{\rm J}}}
\newcommand{\gjup}{\ensuremath{\g_{\rm J}}}

\newcommand{\rjuplong}{\ensuremath{R_{\rm Jup}}}
\newcommand{\mjuplong}{\ensuremath{M_{\rm Jup}}}
\newcommand{\ljuplong}{\ensuremath{L_{\rm Jup}}}
\newcommand{\teffjuplong}{\ensuremath{T_{eff,{\rm Jup}}}}
\newcommand{\rhojuplong}{\ensuremath{\rho_{\rm Jup}}}
\newcommand{\gjuplong}{\ensuremath{\g_{\rm Jup}}}

%% -----------------------------
%% Software
\newcommand{\pack}[1]{\textsc{\lowercase{#1}}}
\newcommand{\prog}[1]{\texttt{\lowercase{#1}}}
\newcommand{\iraf}{\pack{iraf}}
\newcommand{\todcor}{\prog{todcor}}
\newcommand{\xcsao}{\prog{xcsao}}
\newcommand{\daophot}{\pack{daophot}}
\newcommand{\fihat}{\pack{fihat}}
\newcommand{\fistar}{\prog{fistar}}
\newcommand{\fiphot}{\prog{fiphot}}
\newcommand{\grmatch}{\prog{grmatch}}
\newcommand{\grtrans}{\prog{grtrans}}

%% ---------------------------------------
%% References
%\newcommand{\pref}[1]{p.~\pageref{#1}}
%\newcommand{\figr}[1]{Fig.~\ref{fig:#1}}
%\newcommand{\secr}[1]{\mbox{\S\ \ref{sec:#1}}}
%\newcommand{\eqr}[1]{Eq.~\ref{eq:#1}}
%\newcommand{\tabsr}[1]{Tab.~\ref{tab:#1}}
%\newcommand{\tabr}[1]{\mbox{Table~\ref{tab:#1}}}
%\newcommand{\figrp}[1]{Fig.~\ref{fig:#1} on \pref{fig:#1}}
%\newcommand{\secrp}[1]{\S\ref{sec:#1} on \pref{sec:#1}}
%\newcommand{\eqrp}[1]{Eq.~\ref{eq:#1} on \pref{eq:#1}}
%\newcommand{\tabrp}[1]{Tab.~\ref{tab:#1} on \pref{tab:#1}}

\newcommand{\refp}[1]{p.~\pageref{#1}}

\newcommand{\reffig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\refsec}[1]{\mbox{\S\ \ref{sec:#1}}}
\newcommand{\refeq}[1]{Eq.~\ref{eq:#1}}
\newcommand{\reftab}[1]{Tab.~\ref{tab:#1}}

\newcommand{\reffigl}[1]{Figure~\ref{fig:#1}}
\newcommand{\refsecl}[1]{\mbox{Section \ref{sec:#1}}}
\newcommand{\refeql}[1]{Equation~\ref{eq:#1}}
\newcommand{\reftabl}[1]{Table~\ref{tab:#1}}

\newcommand{\reffigp}[1]{\reffig{#1} on \pref{fig:#1}}
\newcommand{\refsecp}[1]{\refsec{#1} on \pref{sec:#1}}
\newcommand{\refeqp}[1]{\refeq{#1} on \pref{eq:#1}}
\newcommand{\reftabp}[1]{\reftab{#1} on \pref{tab:#1}}

%% --------------------------------------
%% Instruments
% 
%% FLWO 1.2 m telescope
\newcommand{\flwof}{\mbox{FLWO 1.2\,m}}

%% FLWO 1.5 m telescope
\newcommand{\flwos}{\mbox{FLWO 1.5\,m}}

%% TopHAT 0.25m telescope
\newcommand{\flwot}{\mbox{TopHAT 0.25\,m}}

%% MMT
\newcommand{\mmt}{\mbox{MMT 6.5\,m}}

%% Spitzer
\newcommand{\ssts}{{\em Spitzer}}
\newcommand{\sstL}{{\em Spitzer Space Telescope}}

%% HST
\newcommand{\hst}{{\em HST}}

%% Wise 1m
\newcommand{\wom}{\mbox{Wise 1\,m}}

\newcommand{\piszkessch}{Konkoly 0.6\,m Schmidt}
\newcommand{\piszkesrcc}{Konkoly 1\,m RCC}


%% --------------------------------------
%% Variable types
%% 
\newcommand{\dscu}{\mbox{$\delta$ Scuti}}
\newcommand{\gdor}{\mbox{$\gamma$ Dor}}

\newcommand{\hj}{hot Jupiter}
\newcommand{\vhj}{very hot Jupiter}

% ---------------------------------------------------------------------
%% Astronomical catalogues

%% HD: 
\newcommand{\hd}[1]{\mbox{HD #1}}

%% BD
\newcommand{\BD}[1]{\mbox{BD #1}}

%% HIP
\newcommand{\hip}[1]{\mbox{HIP #1}}

%% GJ
\newcommand{\gj}[1]{\mbox{GJ #1}}

% ---------------------------------------------------------------------
% Shorthand
\newcommand{\tbn}[1]{\tablenotemark{#1}}

